SLIM: Scalable and Lightweight LiDAR Mapping in Urban Environments

LiDAR point cloud maps are extensively utilized on roads for robot navigation due to their high consistency. However, dense point clouds face challenges of high memory consumption and reduced maintainability for long-term operations. In this study, we introduce SLIM, a scalable and lightweight mapping system for long-term LiDAR mapping in urban environments. The system begins by parameterizing structural point clouds into lines and planes. These lightweight and structural representations meet the requirements of map merging, pose graph optimization, and bundle adjustment, ensuring incremental management and local consistency. For long-term operations, a map-centric nonlinear factor recovery method is designed to sparsify poses while preserving mapping accuracy. We validate the SLIM system with multi-session real-world LiDAR data from classical LiDAR mapping datasets, including KITTI, NCLT, HeLiPR and M2DGR. The experiments demonstrate its capabilities in mapping accuracy, lightweightness, and scalability. Map re-use is also verified through map-based robot localization. Finally, with multi-session LiDAR data, the SLIM system provides a globally consistent map with low memory consumption (~130 KB/km on KITTI).

==> figure-caption/factorgraph.tex <==
\begin{figure}[t]
	\centering
	\includegraphics[width=\linewidth]{figure/CarlaCase.pdf}
	\caption{A case of map merging and the co-visible connection with bird's-eye-view on CARLA simulator.  The source map is from two sub-maps (Session 1 and Session 2, top-left) and a new map (Session 3, top-middle) is merged into the source map. The loop candidates (bold green lines) are provided by GraffMatch, and pruned by PCM and all the remaining loop candidates are reliable. The observations between the keyframes and landmarks are rendered as black lines (only poles are visualized for a clearer visualization). }
	\label{figure:FactorGraph}
\end{figure}
